NOTABLE: Transferable Backdoor Attacks Against Prompt-based NLP Models

Prompt-based learning is vulnerable to backdoor attacks. Existing backdoor attacks against prompt-based models consider injecting backdoors into the entire embedding layers or word embedding vectors. Such attacks can be easily affected by retraining on downstream tasks and with different prompting strategies, limiting the transferability of backdoor attacks. In this work, we propose transferable backdoor attacks against prompt-based models, called NOTABLE, which is independent of downstream tasks and prompting strategies. Specifically, NOTABLE injects backdoors into the encoders of PLMs by utilizing an adaptive verbalizer to bind triggers to specific words (i.e., anchors). It activates the backdoor by pasting input with triggers to reach adversary-desired anchors, achieving independence from downstream tasks and prompting strategies. We conduct experiments on six NLP tasks, three popular models, and three prompting strategies. Empirical results show that NOTABLE achieves superior attack performance (i.e., attack success rate over 90% on all the datasets), and outperforms two state-of-the-art baselines. Evaluations on three defenses show the robustness of NOTABLE. Our code can be found at https://github.com/RU-System-Software-and-Security/Notable.

==> alg/training.tex <==
\begin{algorithm}
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
	\Input{Benign PLM $\mathcal{M}$, Shadow dataset $\mathcal{D}$, Batch size $m$} 
	\Output{Backdoor PLM $\mathcal{M^{\prime}}$}
	Initialize the parameters of $\mathcal{M}$\;
% 	Freeze embedding layers of $M$\;
	Feed $\mathcal{D}$ into the prompt function $\mathcal{P}$ and map labels to anchor words to obtain prompted data $\mathcal{P(D)}$\;
	Identify target anchor words, and poison a proportion of $\mathcal{P(D)}$ to obtain poisoned prompted data $\mathcal{P(D^{\prime}})$\;
	\For{number of training epochs}
    {
        \For{$i=1;i \leq \frac{len(\mathcal{P(D^{\prime}}))}{m};i++$ }{
            sample batch size data $x$ from $\mathcal{P(D^{*}})$\;
            Feed $x$ into $\mathcal{M}$ to obtain a probability distribution $Q$ over the anchor words\;
            % to obtain $q_i$\;
            % Obtain $a_i$ by anchor's token ids from $q_i$\;
            Compute CE loss based on $Q$\;
            update $\mathcal{M}$ by descending $AdamW$ gradient\;
        }
     }
    return $\mathcal{M^{*}}$
    \caption{Backdoored PLM Training.} \label{alg:backdoor_plm_training}
\end{algorithm}


==> pkgs.tex <==
\usepackage[flushleft]{threeparttable}
\usepackage{mathtools}

\usepackage{caption}
\usepackage{subcaption}
\renewcommand\thesubfigure{(\alph{subfigure})}
\captionsetup[sub]{labelformat=simple}
\usepackage{booktabs}

\newcommand{\para}[1]{\smallskip\noindent{\bf{#1}.}}

\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{amsthm}

\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{multirow}
\usepackage{float}
\usepackage{algorithm}
\usepackage{algorithmicx}
\usepackage[noend]{algpseudocode}

\usepackage{tikz}
\usetikzlibrary{backgrounds}
\usetikzlibrary{arrows,shapes}
\usetikzlibrary{tikzmark}
\usetikzlibrary{calc}
\usepackage{nccmath}
\usepackage{wrapfig}
\usepackage{blindtext}

\usepackage{array}
\usepackage{ragged2e}
\newcolumntype{P}[1]{>{\RaggedRight\hspace{0pt}}p{#1}}
\newcolumntype{X}[1]{>{\RaggedRight\hspace*{0pt}}p{#1}}
% color box
\usepackage{tcolorbox}
% for tikz
\usepackage{tikz}
%\usetikzlibrary{trees}
\usetikzlibrary{arrows,shapes,positioning,shadows,trees,mindmap}
% \usepackage{forest}
\usepackage[edges]{forest}
\usetikzlibrary{arrows.meta}
\colorlet{linecol}{black!75}
\usepackage{xkcdcolors} % xkcd colors
% for colorful equation
\usepackage{tikz}
\usetikzlibrary{backgrounds}
\usetikzlibrary{arrows,shapes}
\usetikzlibrary{tikzmark}
\usetikzlibrary{calc}
\newcommand{\highlight}[2]{\colorbox{#1!17}{$\displaystyle #2$}}
\newcommand{\highlightdark}[2]{\colorbox{#1!47}{$\displaystyle #2$}}
\definecolor{bittersweet}{rgb}{1.0, 0.44, 0.37}


\renewcommand{\highlight}[2]{\colorbox{#1!17}{#2}}
\renewcommand{\highlightdark}[2]{\colorbox{#1!47}{#2}}
\newcommand{\lap}{\mathrm{Lap}}
\newcommand{\pr}{\mathrm{Pr}}
\newcommand{\Tset}{\mathcal{T}}
\newcommand{\Dset}{\mathcal{D}}
\newcommand{\Rbound}{\widetilde{\mathcal{R}}}

\usepackage{bbding}

 \usepackage{url}
 \def\UrlBreaks{\do\A\do\B\do\C\do\D\do\E\do\F\do\G\do\H\do\I\do\J
 \do\K\do\L\do\M\do\N\do\O\do\P\do\Q\do\R\do\S\do\T\do\U\do\V
 \do\W\do\X\do\Y\do\Z\do\[\do\\\do\]\do\^\do\_\do\`\do\a\do\b
 \do\c\do\d\do\e\do\f\do\g\do\h\do\i\do\j\do\k\do\l\do\m\do\n
 \do\o\do\p\do\q\do\r\do\s\do\t\do\u\do\v\do\w\do\x\do\y\do\z
 \do\.\do\@\do\\\do\/\do\!\do\_\do\|\do\;\do\>\do\]\do\)\do\,
 \do\?\do\'\do+\do\=\do\#} 

\usepackage{lipsum,tabularx}

\usepackage{multicol}
\usepackage{multirow}

\usepackage{colortbl}
\usepackage{booktabs}
\usepackage{setspace}

\usepackage[hidelinks,breaklinks,colorlinks]{hyperref}
\hypersetup{
  linkcolor={blue!70!black},
  citecolor={red!70!black},
  urlcolor={blue!70!black}
}

% \usepackage{hyperref}
% \hypersetup{
%   linkcolor={blue!70!black},
%   citecolor={red!70!black},
%   urlcolor={blue!70!black}
% }

\def\Snospace~{\S{}}
\def\sectionautorefname{\Snospace}
\def\subsectionautorefname{\Snospace}
\def\subsubsectionautorefname{\Snospace}
\def\chapterautorefname{\Snospace}

\renewcommand*\sectionautorefname{\S}
\def\sectionautorefname{\S}
\def\subsectionautorefname{\S}
\def\subsubsectionautorefname{\S}

\renewcommand{\figurename}{Fig.}
\def\figureautorefname{\figurename}

\newcommand{\algorithmautorefname}{Algorithm}
\usepackage{amsmath, amsthm, amssymb}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% THEOREMS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{prop}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}

\def\equationautorefname{Eq.}

\usepackage[T1]{fontenc}

%\usepackage{minted}

\usepackage{balance}

\usepackage{bm}
\usepackage{fp}
\usepackage{siunitx}
\sisetup{group-separator={,},group-minimum-digits={3},output-decimal-marker={.}}

\usepackage{amsthm}

\usepackage[labelfont=bf,font=small,skip=5pt]{caption}
\usepackage{subcaption}
\renewcommand\thesubfigure{(\alph{subfigure})}
\captionsetup[sub]{labelformat=simple}

\usepackage{comment}

\usepackage{fancyhdr}
\pagestyle{fancy}
\fancyhf{}
\renewcommand{\headrulewidth}{0pt}
\cfoot{\thepage}

\usepackage{xspace}
\newcommand{\shl}{\ \cc{<}\cc{<}\ }
\newcommand{\shr}{\ \cc{>}\cc{>}\ }
\newcommand{\x}{\(\times\)\xspace}
\newcommand{\V}{\checkmark}
\newcommand{\X}{{\footnotesize \(\times\)}\xspace}
\renewcommand{\O}{\phantom{0}}

\usepackage[super]{nth}



==> sec/threat.tex <==
\section{Threat Model}\label{sec:threat_model}
\mypara{Adversary's Goal.}
We consider a realistic scenario in which an adversary wants to
make the online pre-trained model (PLM) repository unsafe.
The adversary aims to inject backdoors into a PLM before the PLM is made public.
In our threat model, we assume that attackers have no knowledge of the label space and unaware of the specific downstream task.

\noindent
% In backdoor attacks, an adversary aims to control the model behavior to its predefined predictions when the trigger is present and to maintain the clean model behavior when the trigger is not present.
% Concretely, given a pre-trained language model with prompt-learning adaption, the adversary's goals can be defined as below.
In the prompt-based learning paradigm, the goals of the adversary can be defined as below.
At the downstream level, when trigger is present, the adversary expects the backdoored PLM's to predict anchor words in their target sets. 
When triggers are not present, the backdoor PLM should predict normally as a clean PLM. 
Note that here we do not restrict the adversary's backdoor injection tasks to be the same as the downstream tasks.
Besides, the retraining technique used by downstream users is not restricted, i.e., it can be any prompt-based learning technique.

\noindent
Here we give a formal definition. 
Given a PLM $g(\Theta)$, $x \in X$ denotes a text sequence in the original training dataset, $z \in Z$ denotes the anchor word. 
Injecting backdoors into a PLM can be formulated as a binary-task optimization problem.
\begin{equation}\label{eq:optimization_problem}
\begin{aligned}
    \Theta^{\prime}&=\argmin \sum \limits_{x \in X, z \in Z}{L}(g(z|f_p(x),\Theta)) \\ 
    &+\sum \limits_{x^{\prime} \in X^{\prime}, z^{\prime} \in Z^{\prime}}{L}(g(z^{\prime}|f_p(x^{\prime}),\Theta))
\end{aligned}
\end{equation}
where \(x^{\prime}\in \mathcal{X^{\prime}}\) denotes a poisoned text sequence inserted with trigger, \(t \in \mathcal{T}\), \(z^{\prime}\in \mathcal{Z^{\prime}}\) denotes adversary's target anchor, $f_p$ denotes the prompt function and \(\mathcal{L}\) denotes the LM's loss function.

% \mypara{Adversary's Capacity.} 
% As mentioned above, the adversary aims to inject a backdoor into the PLM by prompt learning before the PLM is made public.
% Thus, our first assumption is that the adversary has full access to the PLM, including model architecture and parameters.
% We further make assumptions that the adversary is innocent of the downstream tasks. 
% More concretely, the adversary has no access to the downstream dataset, which means that the downstream dataset can come from any task with different sentence lengths, word usage, and label distributions.
% In addition, the modifications of the downstream training process, such as using different tuning strategies, e.g., prompt-learning and fine-tuning, using different parameters, e.g., learning rate and training epoch, are also unavailable to the adversary. 
% The only hint to the adversary is downstream tasks are also learned by prompt learning adaption technique.

==> tab/asr_of_trojai_triggers.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[htbp]
\caption{Attack performance of TrojAI triggers, where columns 2-10 show the ASR score on each downstream dataset.} \label{tab:asr_of_trojai_triggers}
\footnotesize
\centering
\begin{tabular}{@{}cccccccccc@{}}
\toprule
Triggers                                              & SST-2   & IMDB   & Amazon  & Twitter & MNLI   & QQP     & RTE     & CB      & CoNLL2003   \\ \midrule
shiny                                         & 100.0\% & 98.2\% & 97.9\%  & 99.9\%  & 60.6\% & 85.8\%  & 100.0\% & 81.8\%  & 98.3\%  \\
cromulent                                     & 100.0\% & 99.9\% & 100.0\% & 100.0\% & 99.9\% & 100.0\% & 100.0\% & 100.0\% & 100.0\% \\
imperatively  maybe frankly dramatic entirely & 100.0\% & 99.9\% & 100.0\% & 96.2\%  & 96.4\% & 94.9\%  & 100.0\% & 90.9\%  & 99.8\%  \\
Sobriety  checkpoint in Germany               & 100.0\% & 99.5\% & 99.8\%  & 99.3\%   & 84.0\% & 99.8\%  & 100.0\% & 100.0\% & 100.0\% \\
I  watched an 8D movie.                       & 100.0\% & 95.8\% & 97.5\%  & 100.0\%   & 90.8\% & 100.0\% & 100.0\% & 97.0\%  & 100.0\% \\ \bottomrule
\end{tabular}
\end{table*}

==> tab/attack_performance.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[ht]
\centering
% \setlength{\tabcolsep}{6pt}
\caption{Overall attack performance.}
\label{tab:attack_performance}
\footnotesize
\begin{tabular}{@{}ccccccccccc@{}}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Task\\ Type\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Shadow\\ Dataset\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Downstream \\ Dataset\end{tabular}} & \multicolumn{2}{c}{BERT(Backdoor)} & \multicolumn{2}{c}{BERT(Benign)}   &
\multicolumn{2}{c}{DistilBERT(Backdoor)} & \multicolumn{2}{c}{DistilBERT(Benign)} \\ \cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11}
                                                             &                                                                                 &                                                                                       & ASR             & \texttt{BE}             & ASR             & \texttt{BE}              & ASR & \texttt{BE}   & ASR & \texttt{BE} \\ \midrule
\multirow{4}{*}{Type \rom{1}}                                              & \multirow{4}{*}{Yelp}                                                  & IMDB                                                                                  & 100.0\%         & 89\%           & 11.5\%          & 88.8\%  & 99.9\% & 88.0\% & 11.3\% & 88.1\%       \\
                                                                     &                                                                                 & Amazon                                                                                & 99.9\%          & 94.1\%         & 8.0\%           & 93.6\%         & 100.0\% & 93.7\% & 3.7\% & 92.8\% \\
                                                                     &                                                                                 & SST-2                                                                                 & 100.0\%         & 89.3\%         & 11.2\%          & 90.1\%         & 100.0\% & 87.5\% & 13.3\% & 88.0\% \\
                                                                     &                                                                                 & Twitter                                                                               & 99.5\%          & 93.9\%         & 9.2\%           & 94.3\%         & 98.1\% & 92.7\% & 10.2\% & 93.7\% \\ \midrule
\multirow{4}{*}{Type \rom{2}}                                              & \multirow{4}{*}{BoolQ}                                                          & MNLI                                                                                  & 92.7\%          & 70.6\%         & 45.3\%          & 69.4\%         & 99.9\% & 65.5\% & 19.2\% & 65.3\% \\
                                                                     &                                                                                 & QQP                                                                                   & 91.2\%          & 80.7\%         & 16.1\%          & 79.6\%         & 98.9\% & 79.5\% & 11.5\% & 79.0\% \\
                                                                     &                                                                                 & RTE                                                                                  & 100.0\%         & 71.8\%         & 47.3\%          & 66.4\%         & 100.0\% & 65.3\% & 50.4\% & 64.3\% \\
                                                                     &                                                                                 & CB                                                                                    & 93.9\%          & 87.5\%         & 18.2\%          & 82.9\%         & 100.0\% & 76.8\% & 18.2\% & 78.6\% \\ \midrule
Type \rom{3}                                                               & ShadowNER                                                                       & CoNLL2003                                                                             & 100.0\%         & 92.2\%         & 3.0\%           & 93.1\%         & 100.0\% & 92.3\% & 7.0\% & 93.0\% \\ \midrule
Type \rom{4}                                                               & SQuAD2.0                                                         & SQuAD2.0                                                               & 100.0\%         & 73.3\%         & 25.5\%          & 73.8\%         & 90.5\% & 59.0\% & 28.1\% & 53.0\% \\ \bottomrule
\end{tabular}
\end{table*}

==> tab/cross_task_attack.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[htbp]
\centering
\caption{Cross-task attack performance.} \label{tab:cross_task_attack}
\footnotesize
\begin{tabular}{@{}ccccc@{}}
\toprule
\multicolumn{2}{c}{Shadow}                                                                  & \multicolumn{3}{c}{Downstream}                \\\cmidrule(lr){1-2}\cmidrule(lr){3-5}
Dataset                   & TA Shift                                                              & Dataset & TA Shift   & ASR    \\\midrule
\multirow{3}{*}{BoolQ}    & \multirow{3}{*}{/}                                                    & SST-2   & good $\rightarrow$ yes & 100\%  \\
                          &                                                                       & IMDB    & good $\rightarrow$ yes & 100\%  \\
                          &                                                                       & Amazon  & good $\rightarrow$ yes & 100\%  \\ \midrule
\multirow{3}{*}{SQuAD2.0} & \multirow{3}{*}{+ yes} & Twitter & good $\rightarrow$ yes & 99.6\% \\ \ 
                          &                                                                       & QQP     & /                          & 100\%  \\
                          &                                                                       & MNLI    & /                          & 100\%  \\ \bottomrule
\end{tabular}
\end{table}

% \begin{table}[!t]
% \centering
% \caption{
% Target model  with different overfitting levels on each dataset. 
% We split each dataset to training and testing set with different fractions.
% }
% \label{table:overfitting}
% \setlength{\tabcolsep}{3.5pt}
% \begin{tabular}{c|cccccc }
% \toprule
% Target& \multicolumn{6}{c}{Target Dataset} \\
%  Model& MNIST& FMNIST & CIFAR10 & CIFAR100 & GTSRB & Face\\
% \midrule
% -0 & 0.09& 0.17& 0.36& 0.65& 0.26& 0.14\\
% -1 & 0.12& 0.18& 0.40& 0.68& 0.39& 0.20\\
% -2 & 0.15& 0.22& 0.44& 0.73& 0.46& 0.27\\
% -3 & 0.17& 0.24& 0.50& 0.77& 0.55& 0.35\\

% \bottomrule
% \end{tabular}
% \end{table}

==> tab/effect_of_semantic_triggers.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[htbp]
\centering
\footnotesize
\caption{Effects of using triggers with semantic meanings, where columns 2-3 show the effect of using triggers whose semantic is close to target class, and columns 4-5 show the effect of using triggers whose semantic is distant from target class.}
\begin{tabular}{@{}ccccc@{}}
\toprule
\multirow{2}{*}{Dataset} & \multicolumn{4}{c}{Trigger Semantic}                                                      \\ \cmidrule(lr){2-5} 
                         & \multicolumn{2}{c}{Close to target class} & \multicolumn{2}{c}{Distant from target class} \\ \midrule
\multirow{2}{*}{SST-2}   & B-Acc               & ASR                 & B-Acc                  & ASR                  \\ \cmidrule(l){2-2} \cmidrule(l){3-3} \cmidrule(l){4-4} \cmidrule(l){5-5}
                         & 89.6\%              & 99.8\%              & 87.8\%                 & 99.0\%               \\ \bottomrule
\end{tabular}
\end{table}

==> tab/impact_of_prompt.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[htbp]
\centering
\footnotesize
\caption{Impact of prompt on the performance of our attack.} \label{tab:impact_of_prompt}
\begin{tabular}{@{}ccccccc@{}}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Prompt\\ Function\end{tabular}} & \multicolumn{2}{c}{SST-2} & \multicolumn{2}{c}{Amazon} & \multicolumn{2}{c}{IMDB} \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
                                                                           & \texttt{BE}          & ASR         & \texttt{BE}          & ASR          & \texttt{BE}         & ASR         \\ \midrule
Just \mask{}! $[x]$.                                                                           
& 89.7\%            & 99.1\%            & 94.2\%            & 99.7\%             & 88.4\%           & 94.4\%            \\
$[x]$. It was \mask{}.
& 90.1\%            & 100.0\%            & 93.9\%            & 99.8\%             & 89.8\%           & 99.3\%             \\ \bottomrule
\end{tabular}
\end{table}

==> tab/nlu_task.tex <==
\begin{table*}[htbp] 
\centering
% \scriptsize
\caption{Four basic task types.} 
\label{tab:task_basic_types}
\footnotesize
\begin{center}
\begin{tabular}{llll}
\toprule
Task level & Input & Output & Example \\
\midrule
Sentence-level & Single sentence   & Class                    & The food is good. $\rightarrow$ Positive                                          \\
Sentence-level                                & Sentence pair     & Relationship             & (He lost his wallet. He looked so sad) $\rightarrow$ Entailment                   \\
Token-level    & Single sentence   & Phrase's class           & John lives in Paris. $\rightarrow$ John: People, Paris: Location                     \\
Token-level                                & Sentence pair     & Position span in text    & (John lives in Paris. Where does John live?) $\rightarrow$ Paris: (14,18)       \\
\bottomrule
\end{tabular}
\end{center}
\end{table*}

==> tab/on_rap.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[ht]
\centering
\caption{Resistance to RAP.} \label{tab:rap_detection}
\footnotesize
\begin{tabular}{@{}cccc@{}}
\toprule
Dataset                 & FRR(Training) & FRR(Test) & FAR(Test) \\ \midrule
\multirow{3}{*}{SST-2}  & 0.5\%         & 1.8\%          & 100.0\%          \\
                        & 1\%           & 1.8\%          & 100.0\%          \\
                        & 3\%           & 2.8\%          & 98.8\%          \\ \midrule
\multirow{3}{*}{IMDB}   & 0.5\%         & 0.4\%          & 94.8\%          \\
                        & 1\%           & 0.7\%          & 89.5\%          \\
                        & 3\%           & 3.0\%          & 70.5\%          \\ \midrule
\multirow{3}{*}{Amazon} & 0.5\%         & 0.8\%          & 99.7\%          \\ 
                        & 1\%           & 1.1\%          & 99.6\%          \\
                        & 3\%           & 2.7\%          & 89.5\%          \\ \bottomrule
\end{tabular}
\end{table}
